Fat $b$-Jet Analyses Using Old and New Clustering Algorithms in New Higgs Boson Searches at the LHC

We compare different jet-clustering algorithms in establishing fully hadronic final states stemming from the chain decay of a heavy Higgs state into a pair of the 125 GeV Higgs boson that decays into bottom-antibottom quark pairs. Such 4$b$ events typically give rise to boosted topologies, wherein bottom-antibottom quark pairs emerging from each 125 GeV Higgs boson tend to merge into a single, fat $b$-jet. Assuming Large Hadron Collider (LHC) settings, we illustrate how both the efficiency of selecting the multi-jet final state and the ability to reconstruct from it the masses of all Higgs bosons depend on the choice of jet-clustering algorithm and its parameter settings. We indicate the optimal choice of clustering method for the purpose of establishing such a ubiquitous Beyond the SM (BSM) signal, illustrated via a Type-II 2-Higgs Doublet Model (2HDM).

==> references.tex <==
%\cite{Krohn:2009zg}
\bibitem{Krohn:2009zg}
D.~Krohn, J.~Thaler and L.~T.~Wang,
%``Jets with Variable R,''
JHEP \textbf{06} (2009), 059
doi:10.1088/1126-6708/2009/06/059
[arXiv:0903.0392 [hep-ph]].
%100 citations counted in INSPIRE as of 15 Oct 2020

%\cite{Chakraborty:2020vwj}
\bibitem{Chakraborty:2020vwj}
A.~Chakraborty, S.~Dasmahapatra, H.~Day-Hall, B.~Ford, S.~Jain, S.~Moretti, E.~Olaiya and C.~Shepherd-Themistocleous,
%``Revisiting Jet Clustering Algorithms for New Higgs Boson Searches in Hadronic Final States,''
[arXiv:2008.02499 [hep-ph]].
%1 citations counted in INSPIRE as of 15 Oct 2020

%\cite{Romao:2019dvs}
\bibitem{Romao:2019dvs}
M.~Rom\~ao Crispim, N.~F.~Castro, R.~Pedro and T.~Vale,
%``Transferability of Deep Learning Models in Searches for New Physics at Colliders,''
Phys. Rev. D \textbf{101} (2020) no.3, 035042
doi:10.1103/PhysRevD.101.035042
[arXiv:1912.04220 [hep-ph]].
%3 citations counted in INSPIRE as of 15 Oct 2020

%\cite{Schwartzman:2016jqu}
\bibitem{Schwartzman:2016jqu}
A.~Schwartzman, M.~Kagan, L.~Mackey, B.~Nachman and L.~De Oliveira,
%``Image Processing, Computer Vision, and Deep Learning: new approaches to the analysis and physics interpretation of LHC events,''
J. Phys. Conf. Ser. \textbf{762} (2016) no.1, 012035
doi:10.1088/1742-6596/762/1/012035
%9 citations counted in INSPIRE as of 15 Oct 2020

%\cite{Lin:2018cin}
\bibitem{Lin:2018cin}
J.~Lin, M.~Freytsis, I.~Moult and B.~Nachman,
%``Boosting $H\to b\bar b$ with Machine Learning,''
JHEP \textbf{10} (2018), 101
doi:10.1007/JHEP10(2018)101
[arXiv:1807.10768 [hep-ph]].
%34 citations counted in INSPIRE as of 10 Nov 2020

%\cite{Cogan:2014oua}
\bibitem{Cogan:2014oua}
J.~Cogan, M.~Kagan, E.~Strauss and A.~Schwarztman,
%``Jet-Images: Computer Vision Inspired Techniques for Jet Tagging,''
JHEP \textbf{02} (2015), 118
doi:10.1007/JHEP02(2015)118
[arXiv:1407.5675 [hep-ph]].
%121 citations counted in INSPIRE as of 05 Nov 2020

%\cite{deOliveira:2015xxd}
\bibitem{deOliveira:2015xxd}
L.~de Oliveira, M.~Kagan, L.~Mackey, B.~Nachman and A.~Schwartzman,
%``Jet-images \textemdash{} deep learning edition,''
JHEP \textbf{07} (2016), 069
doi:10.1007/JHEP07(2016)069
[arXiv:1511.05190 [hep-ph]].
%175 citations counted in INSPIRE as of 10 Nov 2020

%\cite{Baglio:2014nea}
\bibitem{Baglio:2014nea}
J.~Baglio, O.~Eberhardt, U.~Nierste and M.~Wiebusch,
%``Benchmarks for Higgs Pair Production and Heavy Higgs boson Searches in the Two-Higgs-Doublet Model of Type II,''
Phys. Rev. D \textbf{90} (2014) no.1, 015008
doi:10.1103/PhysRevD.90.015008
[arXiv:1403.1264 [hep-ph]].
%106 citations counted in INSPIRE as of 03 Nov 2020

%\cite{Alwall:2014hca}
\bibitem{Alwall:2014hca}
J.~Alwall, R.~Frederix, S.~Frixione, V.~Hirschi, F.~Maltoni, O.~Mattelaer, H.~S.~Shao, T.~Stelzer, P.~Torrielli and M.~Zaro,
%``The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations,''
JHEP \textbf{07} (2014), 079
doi:10.1007/JHEP07(2014)079
[arXiv:1405.0301 [hep-ph]].
%5114 citations counted in INSPIRE as of 11 Nov 2020

%\cite{Sjostrand:2007gs}
\bibitem{Sjostrand:2007gs}
T.~Sjostrand, S.~Mrenna and P.~Z.~Skands,
%``A Brief Introduction to PYTHIA 8.1,''
Comput. Phys. Commun. \textbf{178} (2008), 852-867
doi:10.1016/j.cpc.2008.01.036
[arXiv:0710.3820 [hep-ph]].
%5615 citations counted in INSPIRE as of 11 Nov 2020

%\cite{Conte:2012fm}
\bibitem{Conte:2012fm}
E.~Conte, B.~Fuks and G.~Serret,
%``MadAnalysis 5, A User-Friendly Framework for Collider Phenomenology,''
Comput. Phys. Commun. \textbf{184} (2013), 222-256
doi:10.1016/j.cpc.2012.09.009
[arXiv:1206.1599 [hep-ph]].
%359 citations counted in INSPIRE as of 11 Nov 2020

%\cite{Conte:2018vmg}
\bibitem{Conte:2018vmg}
E.~Conte and B.~Fuks,
%``Confronting new physics theories to LHC data with MADANALYSIS 5,''
Int. J. Mod. Phys. A \textbf{33} (2018) no.28, 1830027
doi:10.1142/S0217751X18300272
[arXiv:1808.00480 [hep-ph]].
%36 citations counted in INSPIRE as of 10 Nov 2020

%\cite{Eriksson:2010zzb}
\bibitem{Eriksson:2010zzb}
D.~Eriksson, J.~Rathsman and O.~Stal,
%``2HDMC: Two-Higgs-doublet model calculator,''
Comput. Phys. Commun. \textbf{181} (2010), 833-834
doi:10.1016/j.cpc.2009.12.016
%59 citations counted in INSPIRE as of 15 Oct 2020

%\cite{Bechtle:2013wla}
\bibitem{Bechtle:2013wla}
P.~Bechtle, O.~Brein, S.~Heinemeyer, O.~St\r{a}l, T.~Stefaniak, G.~Weiglein and K.~E.~Williams,
%``$\mathsf{HiggsBounds}-4$: Improved Tests of Extended Higgs Sectors against Exclusion Bounds from LEP, the Tevatron and the LHC,''
Eur. Phys. J. C \textbf{74} (2014) no.3, 2693
doi:10.1140/epjc/s10052-013-2693-2
[arXiv:1311.0055 [hep-ph]].
%429 citations counted in INSPIRE as of 10 Nov 2020

%\cite{Bechtle:2013xfa}
\bibitem{Bechtle:2013xfa}
P.~Bechtle, S.~Heinemeyer, O.~St\r{a}l, T.~Stefaniak and G.~Weiglein,
%``$HiggsSignals$: Confronting arbitrary Higgs sectors with measurements at the Tevatron and the LHC,''
Eur. Phys. J. C \textbf{74} (2014) no.2, 2711
doi:10.1140/epjc/s10052-013-2711-4
[arXiv:1305.1933 [hep-ph]].
%404 citations counted in INSPIRE as of 09 Nov 2020

%\cite{Mahmoudi:2009zz}
\bibitem{Mahmoudi:2009zz}
F.~Mahmoudi,
%``SuperIso v3.0, flavor physics observables calculations: Extension to NMSSM,''
Comput. Phys. Commun. \textbf{180} (2009), 1718-1719
doi:10.1016/j.cpc.2009.05.001
%71 citations counted in INSPIRE as of 05 Nov 2020

%\cite{Cacciari:2008gp}
\bibitem{Cacciari:2008gp}
M.~Cacciari, G.~P.~Salam and G.~Soyez,
%``The anti-$k_t$ jet clustering algorithm,''
JHEP \textbf{04} (2008), 063
doi:10.1088/1126-6708/2008/04/063
[arXiv:0802.1189 [hep-ph]].
%7447 citations counted in INSPIRE as of 11 Nov 2020

%\cite{Cacciari:2011ma}
\bibitem{Cacciari:2011ma}
M.~Cacciari, G.~P.~Salam and G.~Soyez,
%``FastJet User Manual,''
Eur. Phys. J. C \textbf{72} (2012), 1896
doi:10.1140/epjc/s10052-012-1896-2
[arXiv:1111.6097 [hep-ph]].
%3786 citations counted in INSPIRE as of 11 Nov 2020
